Traj-MAE: Masked Autoencoders for Trajectory Prediction

Trajectory prediction has been a crucial task in building a reliable autonomous driving system by anticipating possible dangers. One key issue is to generate consistent trajectory predictions without colliding. To overcome the challenge, we propose an efficient masked autoencoder for trajectory prediction (Traj-MAE) that better represents the complicated behaviors of agents in the driving environment. Specifically, our Traj-MAE employs diverse masking strategies to pre-train the trajectory encoder and map encoder, allowing for the capture of social and temporal information among agents while leveraging the effect of environment from multiple granularities. To address the catastrophic forgetting problem that arises when pre-training the network with multiple masking strategies, we introduce a continual pre-training framework, which can help Traj-MAE learn valuable and diverse information from various strategies efficiently. Our experimental results in both multi-agent and single-agent settings demonstrate that Traj-MAE achieves competitive results with state-of-the-art methods and significantly outperforms our baseline model.

==> no_use.tex <==
% !TEX root = ../submission.tex
\section{Experiments}
\subsection{Datasets.}
%\noindent\textbf{Datasets.}
Argoverse motion forecasting dataset \cite{chang2019argoverse} provides 333K real-world driving sequences, which are sampled at 10Hz, with 2 seconds history and 3 seconds future. The whole dataset is split into train, validation and test sets, with 205942, 39472, and 78143 sequences, respectively.
The Interaction dataset \cite{zhan2019interaction} consists of various highly interactive driving situations, and each trajectory has 1 second history and 3 seconds future sampled at 10Hz. In the multi-agent prediction track, the target is to predict multiple target agents' coordinates and yaw jointly.
The synthetic partition of the TrajNet++ dataset \cite{sadeghian2018trajnet} has 54513 scenes. Given the state of all agents of the past 9 timesteps, the goal is to predict the next 12 timesteps for all agents.
\iffalse
\noindent\textbf{Metrics.}
For the task to predict the ego-agent's future trajectory, we use minADE(k), minFDE(k) and MR(k) to evaluate our method, which are respectively the minimum Average Displacement Error, the minimum Final Displacement Error and the Miss Rate for the top \textit{k} predictions. Considering the multi-agents' future trajectories prediction task, we calculate ego-agent's prediction error and scene-level prediction error as defined by \cite{casas2020implicit} on TrajNet++ dataset. Similarly, MinJointADE, MinJointFDE and MinJointMR are used to calculate multi-agents' prediction error. Cross Collision Rate represents the frequency of collisions happening among the predictions of all agents and Ego Collision Rate represents the collisions happening between ego-agent and others. When only considering those modalities without cross collision, Consistent MinJointMR is calculated as the case's MR.

\noindent\textbf{Implementation Details.}
For pre-training, we use an Adam optimizer \cite{kingma2014adam} with a fixed learning rate 1e-3. We set the same number of training stages as the number of pre-training strategies as shown in Table \ref{table:continual_setting}. When performing continuous pre-training, 
%we consider the multiple strategies we design as equally important, thus 
the number of epochs for each strategy in all training stages adds up to 200.
In terms of the trajectory prediction task, we fine-tune Autobots on three challenging datasets, and utilize Adam \cite{kingma2014adam} as an optimizer. For the Argoverse dataset, we use Autobot-Ego as our baseline model, the initial learning rate is set at 3e-5, and for the Interaction and TrajNet++ datasets, Autobot is used as the baseline model, we set the initial learning rates at 5e-5 and 7e-5, respectively. We anneal the learning rate every 10 epochs by a factor of 2 in the first 50 epochs, and the total training epochs are 150.
%\gy{the term should be consistent} 
The batch size of training and testing of all the above tasks is 64. The Traj-MAE is implemented by PyTorch \cite{paszke2019pytorch} and all experiments can be done on a single V100.
%the experiments are done on a workstation with 6 V100 GPUs.
%\liu{depending on the page limitation, some parts can move to appendix if needed} Jiaze: well noted with thanks!
\fi
\subsection{Experimental Results.}~\label{section:results}
In this subsection, we pre-train and fine-tune the model on the same benchmark to validate the benefit brought by our proposed self-supervised learning method.

\noindent\textbf{Results on Argoverse.}
The trajectory prediction results on Argoverse are reported in Table \ref{table:argo_val} and Table \ref{table:argo_test}.
On the Argoverse validation set, our Traj-MAE decreases the minADE by 15\%, minFDE by 5\% and MR by 17\%. And it decreases minADE, minFDE and MR by 4\%, 4\% and 6\% on the Argoverse test set, respectively.
The performance demonstrates that our Traj-MAE significantly outperforms our baseline method (Autobot-Ego).
Moreover, Our Traj-MAE provides an effective and GPU-friendly pre-training mechanism only pre-trained on a single GPU (V100) in under \emph{48h}.
Different from DenseTNT\cite{gu2021densetnt}, HOME\cite{gilles2021home} and GOHOME\cite{gilles2022gohome}, which adopt optimization algorithm to optimize the MR, we use a simple learnable seed parameters design following Autobots, which allows our network perform a high inference speed on the entire scene with a single forward pass.

\begin{table}[]
\scriptsize
\centering
%resizebox{\columnwidth}{!}{
\begin{tabular}{cccc} \toprule
Method & \hspace{-1.0cm}minADE & \hspace{-0.9cm}minFDE & \hspace{-0.9cm}MR \\ \hline
DESIRE~\cite{lee2017desire} & \hspace{-1.0cm}0.92 & \hspace{-0.9cm}1.77 & \hspace{-0.9cm}0.18 \\
MultiPath~\cite{chai2019multipath} & \hspace{-1.0cm}0.80 & \hspace{-0.9cm}1.68 & \hspace{-0.9cm}0.14 \\
TNT~\cite{zhao2020tnt} & \hspace{-1.0cm}0.73 & \hspace{-0.9cm}1.29 & \hspace{-0.9cm}0.09 \\
LaneRCNN~\cite{zeng2021lanercnn} & \hspace{-1.0cm}0.77 & \hspace{-0.9cm}1.19 & \hspace{-0.9cm}0.08 \\
TPCN~\cite{ye2021tpcn} & \hspace{-1.0cm}0.73 & \hspace{-0.9cm}1.15 & \hspace{-0.9cm}0.11 \\
mmTransformer~\cite{liu2021multimodal} & \hspace{-1.0cm}0.71 & \hspace{-0.9cm}1.15 & \hspace{-0.9cm}0.11 \\
DenseTNT~\cite{gu2021densetnt} & \hspace{-1.0cm}0.82 & \hspace{-0.9cm}1.37 & \hspace{-0.9cm}\textbf{0.07} \\
HiVT\cite{zhou2022hivt} & \hspace{-1.0cm}0.66 & \hspace{-0.9cm}0.96 & \hspace{-0.9cm}0.09 \\ 
DCMS\cite{ye2022dcms} & \hspace{-1.0cm}0.64 & \hspace{-0.9cm}\textbf{0.93} & \hspace{-0.9cm}- \\ 
GANet\cite{wang2022ganet} & \hspace{-1.0cm}0.67 & \hspace{-0.9cm}\textbf{0.93} & \hspace{-0.9cm}- \\ \hline
Autobot-Ego~\cite{girgis2022latent} & \hspace{-1.0cm}0.73 & \hspace{-0.9cm}1.10 & \hspace{-0.9cm}0.12 \\
\textbf{Traj-MAE} & \hspace{-0.3cm}\textbf{0.62} \red{$\downarrow$ 15\%} & \hspace{-0.3cm}1.04 \red{$\downarrow$ 5\%} & \hspace{-0.2cm}0.10 \red{$\downarrow$ 17\%} \\ \toprule
\end{tabular}
%}
\caption{\textbf{Comparison with state-of-the-art methods on the Argoverse validation set}.}
\label{table:argo_val}
\vspace{-10pt}
\end{table}

\noindent\textbf{Results on INTERACTION.}
In Table \ref{table:INTERACTION}, we compare our method with previous approaches on the challenging multi-agent joint interaction problem.
We evaluate our method on the INTERACTION multi-agent track and rank the \textbf{\emph{1st}} result on the leaderboard.
We can observe that Traj-MAE outperforms all other approaches in terms of Consistent MinJointMR, which is the ranking metric.
This metric encourages the model to make consistent predictions.
Therefore, thus the best result on this metric indicates that our Traj-MAE can well capture multi-agents' interaction.
As for other metrics, our model still has competitive results.
%The experimental results demonstrate the advantage of our Traj-MAE, which can better utilize social information and avoid collisions between agents.
Especially, the reductions of 26\% and 30\% in Cross CollisionRate and Ego CollisionRate demonstrate that our Traj-MAE can better utilize social information and avoid collisions between agents.

\noindent\textbf{Results on TrajNet++.}
To demonstrate that our Traj-MAE has the ability to capture the social and temporal information for multi-agent trajectory prediction.
We evaluate our method on the synthetic partition of TrajNet++ dataset, which has a high-level interaction between different agents.
We compare our model with linear extrapolation (Linear), our baseline Autobot,  and its variants: AutoBot-AntiSocial (AutoBot-AS) and AutoBot-Ego.
The experiment results of agent-level metrics and scene-level metrics defined by \cite{casas2020implicit} are reported in Table \ref{table:Traj++}.
%Our Traj-MAE largely improves the baseline by 0.019, 0.034, 0.036 and 0.070 on the four evaluation metrics Ego Agent's minADE, Ego Agent's minFDE, Scene-level minADE, Scene-level minFDE, respectively.
Our Traj-MAE achieves large reductions of 22\%, 27\%, 23\% with respect to Ego Agent's minADE, Scene-level minADE, and Scene-level minFDE respectively.

\subsection{Ablation Studies.}
To investigate the properties of our method, we perform in-depth ablation studies on the Argoverse validation set in this subsection. 
For these experiments, all models share the same experiment settings.
%and evaluation protocol.
We evaluate our models on minADE, minFDE, and miss rate (MR) of the predicted $6$ trajectories.


\begin{table}[]
\scriptsize
\centering
%\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc} \toprule
Method & \hspace{-0.8cm}minADE & \hspace{-0.9cm}minFDE & \hspace{-0.9cm}MR \\ \hline
TNT\cite{zhao2020tnt} & \hspace{-0.8cm}0.94 & \hspace{-0.9cm}1.54 & \hspace{-0.9cm}0.13 \\
LaneRCNN\cite{zeng2021lanercnn} & \hspace{-0.8cm}0.90 & \hspace{-0.9cm}1.45 & \hspace{-0.9cm}0.12 \\
mmTransformer\cite{liu2021multimodal} &\hspace{-0.8cm} 0.84 & \hspace{-0.9cm}1.34 & \hspace{-0.9cm}0.15 \\
GOHOME\cite{gilles2022gohome} & \hspace{-0.8cm}0.94 & \hspace{-0.9cm}1.45 & \hspace{-0.9cm}\textbf{0.11} \\
TPCN\cite{ye2021tpcn} & \hspace{-0.8cm}0.87 & \hspace{-0.9cm}1.38 & \hspace{-0.9cm}0.16 \\
Scene Transformer\cite{ngiam2021scene} & \hspace{-0.8cm}0.80 & \hspace{-0.9cm}1.23 & \hspace{-0.9cm}0.13 \\
MultiPath++\cite{varadarajan2022multipath++} & \hspace{-0.8cm}0.79 & \hspace{-0.9cm}1.21 & \hspace{-0.9cm}0.13        \\
DenseTNT\cite{gu2021densetnt} & \hspace{-0.8cm}0.88 & \hspace{-0.9cm}1.28 & \hspace{-0.9cm}0.13 \\ 
HiVT\cite{zhou2022hivt} & \hspace{-0.8cm}\textbf{0.77} & \hspace{-0.9cm}1.17 & \hspace{-0.9cm}0.13 \\ 
%DenseTNT-LBF\cite{zhong2022aware} & \hspace{-0.8cm}0.85 & \hspace{-0.9cm}1.31 & \hspace{-0.9cm}- \\
Wayformer\cite{nayakanti2022wayformer} & \hspace{-0.8cm}\textbf{0.77} & \hspace{-0.9cm}\textbf{1.16} & \hspace{-0.9cm}0.12 \\\hline
%DCMS\cite{ye2022dcms} & \hspace{-0.8cm}\textbf{0.77} & \hspace{-0.9cm}\textbf{1.14} & \hspace{-0.9cm}\textbf{0.11} \\
%GANet\cite{wang2022ganet} & \hspace{-0.8cm}0.81 & \hspace{-0.9cm}1.16 & \hspace{-0.9cm}0.12 \\ \hline
Autobot-Ego \cite{girgis2022latent} & \hspace{-0.8cm}0.89 & \hspace{-0.9cm}1.41 & \hspace{-0.9cm}0.16 \\
\textbf{Traj-MAE} & \hspace{-0.2cm}0.85 \red{$\downarrow$ 4\%} & \hspace{-0.4cm}1.32 \red{$\downarrow$ 6\%} & \hspace{-0.4cm}0.15 \red{$\downarrow$ 6\%}\\ \toprule
\end{tabular}
%}
\caption{\textbf{Comparison with state-of-the-art methods on the Argoverse test set}.}
\label{table:argo_test}
\vspace{-10pt}
\end{table}

\begin{table*}[!]
\scriptsize
\centering
%\resizebox{\textewidth}{!}{
%\setlength{\tabcolsep}{0.1mm}{
\begin{tabular}{ccccccc} \toprule
Method & MinJointADE & MinJointFDE& MinJointMR & \begin{tabular}[c]{@{}c@{}}\hspace{-0.2cm}Cross\\ \hspace{-0.2cm}CollisionRate\end{tabular} & \begin{tabular}[c]{@{}c@{}}\hspace{-0.2cm}Ego\\ \hspace{-0.2cm}CollisionRate\end{tabular} & \begin{tabular}[c]{@{}c@{}}Consistent\\ MinJointMR\end{tabular} \\ \hline
DenseTNT\cite{gu2021densetnt} & 0.412 & 1.129 & 0.224 & \hspace{-0.2cm}\textbf{0} & \hspace{-0.2cm}0.014 & 0.224 \\
HDGT\cite{jia2022hdgt} & \textbf{0.303} & \textbf{0.958} & 0.194 & \hspace{-0.2cm}0.163 & \hspace{-0.2cm}0.005 & 0.236 \\
THOMAS\cite{gilles2021thomas} & 0.416 & 0.968 & \textbf{0.179} & \hspace{-0.2cm}0.128 & \hspace{-0.2cm}0.011 & 0.252 \\
ReCoG2\cite{mo2020recog} & 0.467 & 1.160 & 0.238 & \hspace{-0.2cm}0.069 & \hspace{-0.2cm}0.011 & 0.268 \\
L-GCN & 0.393 & 1.249 & 0.284 & \hspace{-0.2cm}0.060 & \hspace{-0.2cm}\textbf{0.004} & 0.297 \\
MoliNet & 0.729 & 2.554 & 0.444 & \hspace{-0.2cm}0.075 & \hspace{-0.2cm}0.042 & 0.473 \\ 
mtz & 0.378 & 1.165 & 0.259 & \hspace{-0.2cm}0.077 & \hspace{-0.2cm}0.006 & 0.272 \\\hline
AutoBot\cite{girgis2022latent} & 0.312 & 1.015 & 0.193 & \hspace{-0.2cm}0.043 & \hspace{-0.2cm}0.010 & 0.207 \\
\textbf{Traj-MAE} & \hspace{0.6cm}0.304 \red{$\downarrow$ 3\%} & 0.982 \red{$\downarrow$ 3\%} & 0.185 \red{$\downarrow$ 4\%} & 0.032 \red{$\downarrow$ 26\%}  & 0.007 \red{$\downarrow$ 30\%} & \textbf{0.197} \red{$\downarrow$ 5\%} \\ \toprule
%\textbf{Traj-MAE} & \hspace{0.82cm}0.304 \red{$\downarrow$ 3\%} & \hspace{0.82cm}0.982 \red{$\downarrow$ 3\%} & \hspace{0.82cm}0.185 \red{$\downarrow$ 4\%} & \hspace{0.82cm}0.032 \red{$\downarrow$ 26\%}  & \hspace{0.82cm}0.007 \red{$\downarrow$ 30\%} & \hspace{0.82cm}\textbf{0.197} \red{$\downarrow$ 5\%} \\ \toprule
\end{tabular}
%}
%}
\caption{\textbf{Comparison with state-of-the-art methods on the INTERACTION}.}
\label{table:INTERACTION}
\vspace{-10pt}
\end{table*}


\begin{table}[!]
\centering
\resizebox{\linewidth}{!}{% 
\begin{tabular}{cccc}
\toprule
Model & \begin{tabular}[c]{@{}c@{}}\hspace{-0.8cm}Ego \\ \hspace{-0.8cm}minADE\end{tabular} & \begin{tabular}[c]{@{}c@{}}\hspace{-1cm}Scene \\ \hspace{-1cm}minADE\end{tabular} & \begin{tabular}[c]{@{}c@{}}\hspace{-1cm}Scene \\\hspace{-1cm} minFDE\end{tabular} \\ \hline
Linear\cite{girgis2022latent} & \hspace{-1cm}0.439 & \hspace{-1cm}0.409 & \hspace{-1cm}0.897 \\
AutoBot-AS\cite{girgis2022latent} & \hspace{-1cm}0.196  & \hspace{-1cm}0.316 & \hspace{-1cm}0.632 \\
AutoBot-Ego\cite{girgis2022latent} & \hspace{-1cm}0.098 & \hspace{-1cm}0.214 & \hspace{-1cm}0.431 \\ \hline
AutoBot\cite{girgis2022latent} & \hspace{-1cm}0.095  & \hspace{-1cm}0.128 & \hspace{-1cm}0.234 \\
\textbf{Traj-MAE} & \textbf{0.074} \red{$\downarrow$ 22\%}  & \textbf{0.093} \red{$\downarrow$ 27\%} & \textbf{0.181} \red{$\downarrow$ 23\%} \\ \toprule
\end{tabular}
}
\caption{\textbf{Results on TrajNet++ for a multi-agent forecasting scenario}. Note that we train the model to predict 6 future trajectories.}
\label{table:Traj++}
\vspace{-10pt}
\end{table}


\begin{table*}[!]
\centering
%\resizebox{\textewidth}{!}{% 
\begin{tabular}{c|ccc|ccc|ccc}
\hline
\multirow{2}{*}{Mask Ratio} & \multicolumn{3}{c|}{Social Masking} & \multicolumn{3}{c|}{Temporal Masking} & \multicolumn{3}{c}{Social and Temporal Masking} \\ \cline{2-10} 
 & minADE & minFDE & MR & minADE & minFDE & MR & minADE & minFDE & MR \\ \hline
30 & 0.668 & 1.091 & 0.115 & 0.664 & 1.094 & 0.116 & 0.659 & 1.091 & 0.113 \\
40 & 0.661 & 1.089 & 0.114  & 0.662 & 1.091 & 0.114 & 0.657 & 1.089 & 0.113 \\
50 & \textbf{0.659} & \textbf{1.085} & \textbf{0.112} & 0.658 & 1.087 & 0.113 & 0.652 & 1.083 & 0.112 \\
60 & 0.663 & 1.090 & 0.113 & \textbf{0.653} & \textbf{1.081} & \textbf{0.110} & \textbf{0.650} & \textbf{1.076} & \textbf{0.110} \\
70 & 0.669 & 1.093 & 0.115 & 0.656 & 1.085 & 0.112 & 0.651 & 1.080 & 0.111 \\
80 & 0.673 & 1.096 & 0.116 & 0.669 & 1.090 & 0.114 & 0.657 & 1.085 & 0.114 \\ \hline
\end{tabular}
%} 
\caption{\textbf{Ablation study on masking strategy with different ratios for trajectory reconstruction}. The reported values are the fine-turn results on Argoverse validation set.}
\label{table:ablation_trajectory}
\vspace{-10pt}
\end{table*}



\begin{table*}[!]
\centering
%\resizebox{\textewidth}{!}{% 
\begin{tabular}{c|ccc|ccc|ccc}
\hline
\multirow{2}{*}{Mask Ratio} & \multicolumn{3}{c|}{Point Masking} & \multicolumn{3}{c|}{Patch Masking} & \multicolumn{3}{c}{Block Masking} \\ \cline{2-10} 
 & minADE & minFDE & MR & minADE & minFDE & MR & minADE & minFDE & MR \\ \hline
30 & 0.666 & 1.084 & 0.112 & 0.668 & 1.085 & 0.112 & 0.671 & 1.087 & 0.113 \\
40 & 0.662 & 1.087 & 0.112 & 0.659 & 1.082 & 0.111 & 0.663 & 1.083 & 0.113 \\
50 & 0.659 & 1.082 & 0.110 & 0.657 & 1.081 & 0.112 & \textbf{0.659} & \textbf{1.080} & \textbf{0.112} \\
60 & \textbf{0.653} & \textbf{1.075} & \textbf{0.109} & \textbf{0.655} & \textbf{1.079} & \textbf{0.110} & 0.661 & 1.082 & 0.113 \\
70 & 0.657 & 1.077 & 0.111 & 0.663 & 1.085 & 0.112 & 0.670 & 1.085 & 0.113 \\
80 & 0.659 & 1.080 & 0.111 & 0.669 & 1.087 & 0.114 & 0.675 & 1.090 & 0.115 \\ \hline
\end{tabular}
%}
\caption{\textbf{Ablation study on masking strategy with different ratios for HD map reconstruction}. The reported values are the fine-turn results on Argover validation set.}
\label{table:ablation_map}
\vspace{-10pt}
\end{table*}

\begin{table*}[!]
\centering
%\begin{minipage}{1.0\textwidth}
\begin{subtable}[c]{0.48\textwidth}
\centering
\begin{tabular}{cccc}
\begin{tabular}{cccc}
\hline
      & Min ADE & Min FDE & MR    \\ \hline
S    & 0.659   & 1.085   & 0.112 \\
T    & 0.653   & 1.081   & 0.110 \\
ST    & 0.650   & 1.076   & 0.110 \\
S+T & 0.641   & 1.069   & 0.105\\
T+S  & 0.652  & 1.088   &  0.110\\
S+T+ST & \textbf{0.630}   & \textbf{1.053}  & \textbf{0.103} \\
ST+T+S & 0.654   & 1.090   & 0.112 \\ \hline
\end{tabular}
\end{tabular}
\subcaption{Continual pre-training for \textbf{trajectory reconstruction}.}
\end{subtable}
%\hspace*{0.02\textwidth}
\begin{subtable}[c]{0.48\textwidth}
\centering
\begin{tabular}{cccc}
\hline
      & Min ADE & Min FDE & MR    \\ \hline
Po    & 0.653   & 1.075   & 0.109 \\
Pa    & 0.655   & 1.079   & 0.110 \\
B    & 0.659   & 1.080   & 0.112 \\
Po+Pa & 0.642   & 1.066   & 0.106 \\
Pa+Po &  0.650  & 1.071   &  0.108 \\
Po+Pa+B & \textbf{0.633}   & \textbf{1.055}   & \textbf{0.102} \\
B+Pa+Po & 0.647   & 1.067   & 0.107 \\ \hline
\end{tabular}
\subcaption{Continual pre-training for \textbf{HD map reconstruction}.}
\end{subtable}

\caption{\textbf{Ablation study on continue pre-training framework}. We show the results using different number of strategies and we observe that the order of strategies affects the performance significantly. Note that 'S', 'T', 'ST' represent \emph{social masking}, \emph{temporal masking}, \emph{social and temporal masking} strategy, respectively. 'Po', 'Pa', 'B' represent \emph{point masking}, \emph{patch masking}, \emph{block masking} strategy, respectively.}
%\end{minipage}
\label{Table:continue}
\vspace{-10pt}
\end{table*}

\noindent\textbf{Trajectory Masking Strategy.}
We compare different trajectory masking strategies with different masking ratios in Table \ref{table:ablation_trajectory}. 
When increasing the masking ratio from 30\% to a threshold (50 $\sim$ 60\%), the performances of the three strategies all increase simultaneously. Then the performances degrade when the masking ratio increase from the threshold to 80\%.
Moreover, with various masking ratios, we find that \emph{social and temporal masking} achieves better performance than that of \emph{social masking} and \emph{temporal masking}, especially on minADE and minFDE.
We argue that the \emph{social and temporal masking} strategy enforce the trajectory encoder to capture more valuable temporal and social information and thus make Traj-MAE a challenging framework for self-supervised trajectory prediction.

\begin{figure*}[h!]
    \centering
        \includegraphics[width=\linewidth]{MAE/img/vis_strategy.png}
    %\vspace{-2pt}
    \caption{\textbf{Reconstruction results on historical trajectory and HD map with different masking strategies.} The leftmost side is input, and  the masked input (left) and reconstruction (right) with different masking strategies are shown in the following columns.}
    \label{fig:vis_strategy}
    \vspace{-10pt}
\end{figure*}

\begin{figure*}[!ht]
    \centering
        \includegraphics[width=\linewidth]{MAE/img/vis_ratio.png}
    %\vspace{-2pt}
    \caption{\textbf{Reconstruction results on historical trajectory and HD map with different masking ratios.} The leftmost side is input, and  the masked input (left) and reconstruction (right) with different masking ratios are shown in the following columns.}
    \label{fig:vis_ratio}
    \vspace{-8pt}
\end{figure*}


\noindent\textbf{Map Masking Strategy.}
Table \ref{table:ablation_map} shows the influence of masking strategies with different masking ratios for HD map.
\emph{Point masking} works best for pre-training our map encoder.
%Besides the better fine-tuning accuracy of point and patch masking, 
Besides, point masking and patch masking allow for a higher masking ratio (60\%) compared to block masking, which can provide a more significant speedup benefit.
The best masking ratios for \emph{block masking} is
50\%. We suppose that with the increase of connected masked parts, the mask and reconstruct task is more challenging, and the optimal mask ratio is smaller. 
%The observation on the masking strategy and ratio also aligns with the analysis in previous works\cite{he2022masked,pang2022masked}.


%\noindent\textbf{Network Design.}

\noindent\textbf{Continual Pre-training Strategy.}
In Traj-MAE, one core design is our continual pre-training framework, which effectiveness can be seen in Table \ref{Table:continue}.
First, we find that our continual pre-training framework further improves the network performance than pre-training on a single task.
With continual pre-training, the trajectory encoder can better capture the social and temporal information, and the map encoder can capture the structured information from multiple granularities.
We also ablate traditional continual learning, and multi-task learning with our continual pre-training. The results show that our method outperforms other learning strategies for both trajectory pre-training and map pre-training (see supplementary material).
What's more, we observe that the sequence of the pre-training strategies also could influence the model performance. 
For trajectory encoder pre-training, the best sequence is \emph{social masking $\to$ temporal masking $\to$ social and temporal masking}.
For map encoder pre-training, the best sequence is 
\emph{point masking $\to$ patch masking $\to$ block masking}.
%The observation is aligned with our intuition that \jiaze{???}.


\begin{table}[!]
\centering
\resizebox{\linewidth}{!}{% 
\begin{tabular}{c|cc|cc}
\hline
 & \multicolumn{2}{c|}{Interaction} & \multicolumn{2}{c}{TrajNet++} \\ \cline{2-5} 
\multirow{-2}{*}{Pre-trained} & minADE & minFDE & minADE & minFDE \\ \hline
None & 0.3123 & 1.0148 & 0.128 & 0.234 \\
Argoverse &0.3101  &0.9982  & 0.116 & 0.211 \\
Self & 0.3036 & 0.9818 & 0.093 & 0.181 \\ \hline
\end{tabular}
}
\caption{\textbf{Transfer learning}.}
\label{table:ablation_domain}
\vspace{-8pt}
\end{table}


\noindent\textbf{Transfer Learning.}
We evaluate transfer learning on other datasets using the model pre-trained on Argoverse.
We fine-tune the pre-trained model on Interaction and TrajNet++ and compared it with the model without pre-training and with self pre-training (pre-training and fine-tuning on itself).
As shown in Table \ref{table:ablation_domain}, our Traj-MAE achieved the best result on both datasets with self pre-trained learning, rather than pre-trained on Argoverse.
We argue that the reason could be that compared to the large-scale datasets used in image and video tasks like ImageNet\cite{deng2009imagenet} and Kinetics\cite{carreira2018short}, the pre-training dataset we used (Argoverse) is relatively small which limits the transfer learning ability of our pre-trained model. 
Therefore, we mainly focus on our self-supervised learning framework as well as pre-train and fine-tune the same dataset.




\noindent\textbf{Qualitative Analysis.}
To demonstrate the effectiveness of our Traj-MAE, we visualize the reconstruction results on the Argoverse validation set.
Figure \ref{fig:vis_strategy} illustrates the different masking strategies.
Although social masking is hard for trajectory reconstruction and block masking is hard for map reconstruction, adopting a medium masking ratio with these strategies can achieve good reconstruction results.
We also compare the different temporal masking ratios and point masking ratios in Figure \ref{fig:vis_ratio}.
The models are pre-trained with a masking ratio of 60\%, but it is capable of reconstructing different masking ratios.
Furthermore, our Traj-MAE can produce satisfying reconstructed trajectories and HD maps even under a high masking ratio, which indicates that our Traj-MAE can learn useful high-level representations.







\iffalse
\noindent\textbf{Results on nuScenes.}
\begin{table*}[]
\centering
%\resizebox{\textewidth}{!}{% 
\begin{tabular}{ccccccc} \toprule
Model & minADE(5) & minADE(10) & MR Top5(2m) & MR Top10(2m) & minFDE(1) & Off Road Rate \\ \hline
Trajectron++ & 1.88 & 1.51 & 0.70 & 0.57 & 9.52 & 0.25 \\
CoverNet & 2.62 & 1.92 & 0.76 & 0.64 & 11.36 & 0.13 \\
Physics Oracle & 3.70 & 3.70 & 0.88 & 0.88 & 9.09 & 0.12 \\
WIMP & 1.84 & 1.11 & 0.55 & 0.43 & 8.49 & 0.04 \\
GOHOME & 1.42 & 1.15 & 0.57 & 0.47 & 6.99 & 0.04 \\ \hline
AutoBot & 1.43 & 1.05 & 0.66 & 0.45 & 8.66 & 0.03 \\
\textbf{Traj-MAE} & 1.41 & 1.00 & 0.60 & 0.38 & 7.96 & 0.03 \\ \toprule
\end{tabular}
%}
\caption{\textbf{Comparison with state-of-the-art methods on the nuScenes}.}
\label{table:nuscenes++}
\end{table*}

The nuScenes dataset \cite{caesar2020nuscenes} contains 700 training scenes and 150 validation scenes, with 32186 training samples and 9041 validation samples, respectively. The goal of this dataset is to predict the 6 seconds future trajectory sampled at 2Hz given the past up to 2 seconds trajectory sampled at 2 Hz.

\begin{figure*}[!ht]
    \centering
    \begin{minipage}{1.0\textwidth}
        \begin{minipage}{0.03\textwidth}
            \begin{center}
                \rotatebox{90}{Trajectory}
            \end{center}
        \end{minipage}
    \begin{minipage}{0.96\textwidth}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_label0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
    \end{minipage}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
    \begin{minipage}{0.03\textwidth}
        \begin{center}
        \rotatebox{90}{Map}
        \end{center}
    \end{minipage}
    \begin{minipage}{0.96\textwidth}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_label0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
    \end{minipage}
    \end{minipage}
    \begin{minipage}{1.0\textwidth}
    \begin{minipage}{0.03\textwidth}
        \begin{center}
        \rotatebox{90}{Map}
        \end{center}
    \end{minipage}
    \begin{minipage}{0.96\textwidth}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_label0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
    \end{minipage}
    \end{minipage}
    \begin{minipage}{1.0\textwidth}
    \begin{minipage}{0.03\textwidth}
        \begin{center}
        \rotatebox{90}{Map}
        \end{center}
    \end{minipage}
    \begin{minipage}{0.96\textwidth}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_label0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.13\linewidth]{MAE/img/v3/map_pred0_0.jpg}
    \end{minipage}
    \end{minipage}
    \vspace{-2pt}
    \caption{Vis masking ratio and strategy.\jiaze{figures to be changed}}\
    \label{fig:vis}
    %\vspace{-8pt}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \begin{minipage}{1.0\textwidth}
        \begin{minipage}{0.03\textwidth}
            \begin{center}
                \rotatebox{90}{Trajectory}
            \end{center}
        \end{minipage}
    \begin{minipage}{0.96\textwidth}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_label0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
    \end{minipage}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
    \begin{minipage}{0.03\textwidth}
        \begin{center}
        \rotatebox{90}{Map}
        \end{center}
    \end{minipage}
    \begin{minipage}{0.96\textwidth}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_label0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
    \end{minipage}
    \end{minipage}
   
    \vspace{-2pt}
    \caption{Vis masking strategy.\jiaze{figures to be changed}}\
    \label{fig:vis}
    \vspace{-8pt}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \begin{minipage}{1.0\textwidth}
        \begin{minipage}{0.03\textwidth}
            \begin{center}
                \rotatebox{90}{Trajectory}
            \end{center}
        \end{minipage}
    \begin{minipage}{0.96\textwidth}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_label0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
    \end{minipage}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
    \begin{minipage}{0.03\textwidth}
        \begin{center}
        \rotatebox{90}{Map}
        \end{center}
    \end{minipage}
    \begin{minipage}{0.96\textwidth}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_label0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_mask0_0.jpg}
        \includegraphics[width=0.1371\linewidth]{MAE/img/v3/map_pred0_0.jpg}
    \end{minipage}
    \end{minipage}
   
    \vspace{-2pt}
    \caption{Vis masking ratio.\jiaze{figures to be changed}}\
    \label{fig:vis2}
    %\vspace{-8pt}
\end{figure*}

\fi

